SIC-free Multicast Scheduling for Multi-antenna Coded Caching

Multi-antenna coded caching (CC) with multicast beamforming typically relies on a complex successive interference cancellation (SIC) structure to decode a superposition of multiple streams received by each user. Signal-level CC schemes require the regeneration and cancellation of interfering signals at the physical layer of each receiver, which complicates practical implementations. To address this, we propose a bit-level multicast scheduling scheme enabling linear, SIC-free decoding of parallel streams by repeatedly transmitting data terms with linearly independent coefficients. Two reference strategies and a novel sparse strategy are considered for constructing the coefficient matrix. The reference cases include the random strategy, which lacks control over matrix construction, and the equal-distant strategy, which balances users' interference and data terms equally. In contrast, the sparse strategy minimizes the number of multicast streams transmitted in parallel during each interval. This approach simplifies both the decoding process and the beamforming design by decoupling the desired data terms for each user and reducing the number of SINR constraints, respectively. To further enhance the symmetric rate, a successive projection algorithm is applied to exploit channel properties and optimize user ordering. With the coefficient matrix and optimized user ordering in place, multicast beamformers are devised to aggregate desired data from relevant multicast streams. Numerical simulations validate the effectiveness of the sparse strategy and user scheduling, demonstrating significant gains in symmetric rate.

==> Figs/DoF_WSA.tex <==
TxAntenna	dofG2	dofG4	dofG6	dofG8	dofG10	dofG12	dofG14
4	8	12	0	0	0	0	0
6	10	12	18	0	0	0	0
8	12	16	18	24	0	0	0
10	14	16	18	24	30	0	0
12	16	20	24	24	30	36	0
14	18	20	24	24	30	36	42


==> Figs/DoF_prop.tex <==
TxAntenna	dofG2	dofG4	dofG6	dofG8	dofG10	dofG12	dofG14	dofG16	dofG18	dofG20
0   0   0   0   0   0   0   0   0   0   0
4	8	12	12	12	12	12	12	12	12	12
8	12	16	24	24	24	24	24	24	24	24
12	16	20	25	32	36	36	36	36	36	36
16	20	24	30	35	40	48	48	48	48	48
20	24	28	36	40	45	48	56	60	60	60
24	0	0	0	0	0	0	0	0	0	0


==> Figs/data.tex <==
SNR	RsymLG32K3t1ISITcov	RsymLG32K3MMSESIC			RsymLG32K3LMMSE		RsymLG42K3t1ISITcov			RsymLG42K3MMSESIC			RsymLG42K3LMMSE			RsymLG32K3LMMSEKKT			RsymLG32K3ZF		RsymLG42K3LMMSEKKT			RsymLG64K420LMMSEKKT			RsymLG74K420LMMSEKKT			RsymLG73K420LMMSEKKT			RsymLG63K420LMMSEKKT			RsymLG42K3ZF			RsymL2G2K2t1cov		RsymLMMSEmultistreamL2G2K2t1				RsymLMMSEsinglestreamL2G2K2t1				RsymLMMSEmultistreamL8G4K3t1				RsymCovL8G4K3t1			RsymLMMSEsinglestreamL8G4K3t1				RsymproposedL8G4K4LMMSE				RsymCovL5G4K3t1			RsymproposedLMMSEL5G4K3t1				RsymproposedcovL6G4t2omg4				RsymproposedLMMSEL2G2omg2t1unicasting					RsymproposedCovL2G2omg2t1unicasting					RsymproposedLMMSEL2G2t1omg2	
																																																																																						
0	5.3365	5.155871462			4.286304845		6.368072742			6.295184266			5.366			4.445386289			1.014394465		5.612811071			14.72973225			16.05390468			12.86568453			11.7813			2.0687			3.6949		3.6324					4.0999				13.1967				13.8776			13.1158				13.4936			10.8459			10.1912				18.4667					2.3698					2.8452					2.840568037
5	10.1285	9.627746908			7.546404254		11.90574618			11.57479304			10.2109			8.07592709			2.744632086		10.50570254			27.43508453			29.78830284			23.97615411			21.5379			5.288			6.811		6.669					7.0231				23.4761				25.2802			22.1641				24.9845			19.8351			18.4914				34.3507					4.5581					5.528					5.464228094
10	16.5253	15.52595966			12.42912228		19.35609748			18.89725902			17.1813			13.00316962			6.391043185		17.26994241			44.74465665			47.90019689			39.63979366			35.6726			11.2387			11.0363		10.8893					10.413				36.9815				40.3851			32.4828				40.6831			31.9366			29.0468				55.838					7.5184					9.2799					9.045829524
15	24.0321	22.48949621			18.68081926		28.32135207			27.7317032			25.6506			18.57993309			12.44784526		25.82016812			64.9039887			68.47440945			58.6044018			53.2958			19.7153			16.3266		16.1615					13.999				53.7595				58.2191			43.3038				59.5164			46.4542			40.6405				81.1861					10.9255					14.1744					13.79933789
20	32.4362	30.26114845			25.73387483		38.36197593			37.48632488			35.284			25.51354743			20.62635136		35.73827386			86.28193517			89.95075643			79.39695807			73.2548			29.7273			22.5407		22.4					17.6551				73.0311				78.225			54.252				80.2317			62.3754			52.5488				108.8675					14.5148					20.1533					19.72999638
25	41.6948	38.59334415			33.68214794		49.01941028			47.87352765			45.6354			33.69018903			30.22308829		46.30414142			108.034779			111.710456			100.8427299			94.4109			40.4233			29.3885		29.2652					21.3349				93.7875				99.533			65.1097				101.6557			78.8102			64.3329				138.6481					18.1597					26.894					26.46651276
30	51.7005	47.56752368			42.96937048		59.94510013			58.61208239			56.326			42.75436618			40.60689773		57.1252819			129.0867536			132.808216			122.3691413			114.3688			51.372			36.561		36.4331					25.0025				115.0608				121.4015			75.4295				122.9313			95.3402			75.5885				170.1896					21.7405					34.0278					33.59691835


==> Figs/dataJ.tex <==
SNR	RsymLG32K3t1ISITcov	RsymLG32K3MMSESIC			RsymLG32K3LMMSE		RsymLG42K3t1ISITcov			RsymLG42K3MMSESIC			RsymLG42K3LMMSE			RsymLG32K3LMMSEKKT			RsymLG32K3ZF		RsymLG42K3LMMSEKKT			RsymLG64K420LMMSEKKT			RsymLG74K420LMMSEKKT			RsymLG73K420LMMSEKKT			RsymLG63K420LMMSEKKT			RsymLG42K3ZF			RsymL2G2K2t1cov		RsymLMMSEmultistreamL2G2K2t1				RsymLMMSEsinglestreamL2G2K2t1				RsymLMMSEmultistreamL8G4K3t1				RsymCovL8G4K3t1			RsymLMMSEsinglestreamL8G4K3t1				RsymproposedL8G4K4LMMSE				RsymCovL5G4K3t1			RsymproposedLMMSEL5G4K3t1				RsymproposedcovL6G4t2omg4				RsymproposedLMMSEL2G2omg2t1unicasting					RsymproposedCovL2G2omg2t1unicasting					RsymproposedLMMSEL2G2t1omg2			RsymproposedCovL3G2omg3t1unicasting					RsymproposedCovL4G2omg3t1unicasting					RsymCovL5G4K3t1Unicasting				RsymproposedLMMSEL6G4t2omg4DoF15					RsymproposedcovL8G4t1omg3Unicasting					RsymproposedCovLG64t2K4unicast					RsymLG32K3LMMSEunicast				RsymproposedLMMSEL6G4t2omg4DoF16					RsymproposedLMMSEL6G4t2omg4DoF12		
																																																																																																																																
0	5.3365	5.155871462			4.286304845		6.368072742			6.295184266			5.366			4.445386289			1.014394465		5.612811071			14.72973225			16.05390468			12.86568453			11.7813			2.0687			3.6949		3.6324					4.0999				13.1967				13.8776			13.1158				13.4936			10.8459			10.1912				16.41483641					2.3698					2.8452					2.840568037			4.0611					4.883					7.8161				13.0986078					10.2628					9.79981515				3.858110047					11.34949					14.24863856	
5	10.1285	9.627746908			7.546404254		11.90574618			11.57479304			10.2109			8.07592709			2.744632086		10.50570254			27.43508453			29.78830284			23.97615411			21.5379			5.288			6.811		6.669					7.0231				23.4761				25.2802			22.1641				24.9845			19.8351			18.4914				30.53393547					4.5581					5.528					5.464228094			7.9493					9.3396					14.9116				23.53900476					19.4142					19.33486659				7.517958808					20.40157					26.90414216	
10	16.5253	15.52595966			12.42912228		19.35609748			18.89725902			17.1813			13.00316962			6.391043185		17.26994241			44.74465665			47.90019689			39.63979366			35.6726			11.2387			11.0363		10.8893					10.413				36.9815				40.3851			32.4828				40.6831			31.9366			29.0468				49.63374893					7.5184					9.2799					9.045829524			13.3102					15.6434					25.0148				38.7980232					32.5012					33.7809236				12.52880151					32.88338					44.13482224	
15	24.0321	22.48949621			18.68081926		28.32135207			27.7317032			25.6506			18.57993309			12.44784526		25.82016812			64.9039887			68.47440945			58.6044018			53.2958			19.7153			16.3266		16.1615					13.999				53.7595				58.2191			43.3038				59.5164			46.4542			40.6405				72.16540523					10.9255					14.1744					13.79933789			19.9162					23.8218					37.9975				58.87593995					48.629					52.83166035				18.67212977					49.21804					64.22364825	
20	32.4362	30.26114845			25.73387483		38.36197593			37.48632488			35.284			25.51354743			20.62635136		35.73827386			86.28193517			89.95075643			79.39695807			73.2548			29.7273			22.5407		22.4					17.6551				73.0311				78.225			54.252				80.2317			62.3754			52.5488				96.77110195					14.5148					20.1533					19.72999638			27.6963					33.4436					53.272				82.27589787					66.9694					74.90136182				25.50081528					68.97584					85.56824545	
25	41.6948	38.59334415			33.68214794		49.01941028			47.87352765			45.6354			33.69018903			30.22308829		46.30414142			108.034779			111.710456			100.8427299			94.4109			40.4233			29.3885		29.2652					21.3349				93.7875				99.533			65.1097				101.6557			78.8102			64.3329				123.242794					18.1597					26.894					26.46651276			36.5683					43.988					69.5993				107.8376535					87.5746					98.7515878				32.96611751					92.07225					107.2911705	
30	51.7005	47.56752368			42.96937048		59.94510013			58.61208239			56.326			42.75436618			40.60689773		57.1252819			129.0867536			132.808216			122.3691413			114.3688			51.372			36.561		36.4331					25.0025				115.0608				121.4015			75.4295				122.9313			95.3402			75.5885				151.2796549					21.7405					34.0278					33.59691835			45.9995					54.6683					85.8244				134.2028653					108.5545					124.1614733				40.67000418					117.8556					128.4987429	
35																																																																																																							160.3418567										150.1559986									145.1262					147.7928479	
40																																																																																																							185.3353853										176.4401799									172.5147					163.401274	

==> Figs/dataJDoF.tex <==
SNR		RsymproposedLMMSEL6G4t2omg4DoF15					RsymproposedCovLG64t2K4unicast					RsymproposedLMMSEL6G4t2omg4DoF16					RsymproposedLMMSEL6G4t2omg4DoF12					RsymproposedcovL6G4t2omg4				RsymproposedLMMSEL6G4t2omg4DoF16Grouping		
0			13.0986078					9.79981515					11.34949					14.24863856					16.41483641			12.51846182		
5			23.53900476					19.33486659					20.40157					26.90414216					30.53393547			22.21561976		
10			38.7980232					33.7809236					32.88338					44.13482224					49.63374893			35.60168262		
15			58.87593995					52.83166035					49.21804					64.22364825					72.16540523			52.56486492		
20			82.27589787					74.90136182					68.97584					85.56824545					96.77110195			72.55114148		
25			107.8376535					98.7515878					92.07225					107.2911705					123.242794			95.73101701		
30			134.2028653					124.1614733					117.8556					128.8987429					151.2796549			121.5245181		
35			160.3418567					150.1559986					145.1262					150.5574					180.1930395			148.9207		
40			185.3353853					176.4401799					174.0314					172.6427					209.4766862			176.7653		


==> Figs/data_Plot1J.tex <==
SNR		RsymLG42K2t0MIMOUnicast			RsymLG42K3t0MIMOUnicast			RsymLG42K4t0MIMOUnicast			RsymLG44K2t1MIMOMulticast			RsymLG41K4t0MIMOUnicast			RsymLG41K5t1MIMOMulticast				RsymLG44K2t0MIMOMulticast				RsymLG42K3t1MIMOMulticast	
																										
0			3.609143706			3.831366754			3.788106685			8.432480659			2.593804317			4.146089997				5.674016394				6.36807274
5			6.389178313			7.146762946			7.226694885			15.13449178			4.738357036			7.762649015				10.38660141				11.90574619
10			9.940045125			11.45468669			12.16106662			24.17553189			7.577245944			12.63556173				16.2269351				19.35609748
15			14.21201437			16.27030372			18.09999176			35.06376109			11.27588789			18.91018625				22.57677916				28.32135207
20			19.20715816			21.24552112			24.46716844			47.492695			15.95214963			26.65520527				29.03434725				38.36197593
25			25.01281006			26.15783114			30.93460437			61.03339456			21.48182592			35.54716734				35.18208212				49.01941029
30			30.94294126			30.99439917			37.22997939			75.22972257			27.59050782			45.01696107				41.6696				59.94510013
35			37.26134518			35.27326354			42.95331617			89.75323113			34.01264417			54.61032636				48.1588				70.96863935
40			43.58667678			39.48470976			48.58089115			104.4201451			40.57485718			64.0936031				54.5827				82.02035419


==> Figs/data_Plot1_Javad.tex <==
SNR	        	Linear			        beta-scheme									
0				0.8473					0.8565
5			    1.6118				    1.6383
10			    2.6944					2.7329	
15			    4.0867					4.1427	
20			    5.7162				    5.7959
25			    7.5173					7.6163
30			    9.4435				    9.5567
35			    11.4651					11.5888
40			    13.5534			        13.6840
45              15.6848                 15.8206
50              17.8444                 17.9839


    


==> Figs/data_Plot2J.tex <==
SNR	RsymLG42K3t1	RsymLG42K4t1	RsymLG42K5t1	RsymLG32K3t1	    RsymLG32K4t1	RsymLG32K2t1	RsymLG32K3LMMSE	RsymLG42K3LMMSE	RsymLG42K3t1WSAZFUnicast		RsymLG32K2t1WSAZFUnicast	
												
0	6.368	6.4835	6.4895	5.3364	5.3014	4.8047	4.286304845	5.366	2.970622533		2.143022131	
5	11.9051	12.2979	12.1508	10.1282	10.105	8.6826	7.546404254	10.2109	6.438479039		4.420501449	
10	19.3557	19.88	19.2401	16.5233	16.6818	14.0075	12.42912228	17.1813	12.0213435		7.885372607	
15	28.3209	28.2528	28.9142	24.0291	24.1823	20.4462	18.68081926	25.6506	19.9216751		12.67259089	
20	38.3617	36.6317	38.3004	32.4269	31.8489	27.4743	25.73387483	35.284	29.5694723		18.62366488	
25	49.019	44.6427	47.5525	41.6848	39.3423	34.7368	33.68214794	45.6354	40.10652076		25.34656728	
30	59.945	52.3203	56.4409	51.6823	46.5181	42.0801	42.96937048	56.326	50.99824058		32.45275667	
												


==> Figs/data_Plot2_Javad.tex <==
SNR	       	Linear			        Linear-ZF   Signal-level-eq Signal-level									
0			0.6469					0.3092         0.1670          0.2470
5			1.3179				    0.8052         0.4616          0.6603
10			2.3129					1.7793	       1.1076          1.5090
15			3.7133					3.3024	       2.2398          2.8939
20			5.5292				    5.2820         3.8670          4.7596
25			7.6733					7.5479         5.8861          6.9534
30			10.0132				    9.9538         8.1559          9.3240
35			12.4444					12.4160        10.5575         11.7721
40			14.9122			        14.8979        13.0167         14.2491
45          17.3938                 17.3863        15.4974         16.7359
50          19.8809                 19.8768        17.9853         19.2258


    

   
 
  

==> Figs/data_Plot3_Javad.tex <==
SNR	       	Linear	  MJ-Signal     Linear-ZF   Signal-level-eq  Signal-level									
0			0.7135	    0.5968		0.1132         0.0452          0.0830
5			1.3473		1.1203		0.3190         0.1345          0.2397
10			2.2018		1.7750		0.7941	       0.3674          0.6211
15			3.3023		2.5717		1.6784	       0.8763          1.3774
20			4.6425		3.5982	    3.0033         1.7811          2.5795
25			6.1743		4.9267		4.6739         3.1054          4.1624
30			7.8579		6.5415      6.5590         4.7637          5.9955
35			9.6641		8.3653		8.5561         6.6350          7.9658
40			11.5635	    10.3221     10.6030        8.6220          10.0012
45          13.5283     12.3524     12.6693        10.6635         12.0631
50          15.5362     14.4160     14.7423        12.7275         14.1346
    





==> Figs/data_Plot4J.tex <==
SNR		RsymLG42K3t1ISITcov			RsymLG42K3LMMSEMC			RsymLG32K3t1ISITcov			RsymLG32K3LMMSEMC			RsymLG32K3LMMSEUC			RsymLG42K3LMMSEUC				RsymLMMSEmultistreamL2G2K2t1					RsymproposedLMMSEL2G2omg2t1unicasting			RsymproposedLMMSEL2G2t1omg2			RsymproposedCovL2G2omg2t1unicasting		RsymproposedCovL4G2omg3t1unicasting		RsymL2G2K2t1cov	
																																					
0		6.368072742			5.366			5.3365			4.286304845			3.858110047				4.715927984			3.6324					2.3698				2.840568037		2.8452		4.883		3.6949	
5		11.90574618			10.2109			10.1285			7.546404254			7.517958808				8.989981409			6.669					4.5581				5.464228094		5.528		9.3396		6.811	
10		19.35609748			17.1813			16.5253			12.42912228			12.52880151				14.88559033			10.8893					7.5184				9.045829524		9.2799		15.6434		11.0363	
15		28.32135207			25.6506			24.0321			18.68081926			18.67212977				22.55882508			16.1615					10.9255				13.79933789		14.1744		23.8218		16.3266	
20		38.36197593			35.284			32.4362			25.73387483			25.50081528				31.77886047			22.4					14.5148				19.72999638		20.1533		33.4436		22.5407	
25		49.01941028			45.6354			41.6948			33.68214794			32.96611751				42.04392012			29.2652					18.1597				26.46651276		26.894		43.988		29.3885	
30		59.94510013			56.326			51.7005			42.96937048			40.67000418				52.82441351			36.4331					21.7405				33.59691835		34.0278		54.6683		36.561	


==> Figs/data_Plot4_Javad.tex <==
%SNR	       	Linear	  Linear-ZF         SIC       SIC-ZF	 NO-CC	   NO-CC-ZF					
%0			0.6947	   0.0966         0.9154      0.1635    0.4922      0.0507
%5			1.3343	   0.2814         1.7213      0.4748    0.9335      0.1523
%10			2.2072	   0.7341	      2.8001      1.2302    1.5389      0.4223
%15			3.3175	   1.6222	      4.1944      2.6771    2.2982      1.0079
%20			4.6421	   2.9907         5.9318      4.8113    3.1808      1.9556
%25			6.1376	   4.7239         7.9398      7.3279    4.1535      3.1073
%30			7.7782	   6.6609         10.0977     9.8741    5.1946      4.2868
%35			9.5471	   8.6875         12.2967     12.2435   6.2779      5.4354
%40			11.4202	   10.7473        14.4668     14.4559   7.3726      6.5550
%45          13.3719    12.8182        16.5916     16.5891   8.4633      7.6562
%50          15.3776    14.8927        18.6917     18.6797   9.5476      8.7454





SNR	       	Linear	  Linear-ZF         SIC       SIC-ZF	 NO-CC	   NO-CC-ZF					
0			0.7135	   0.1132         0.9333      0.1909    0.4922      0.0507
5			1.3473	   0.3190         1.7484      0.5380    0.9335      0.1523
10			2.2018	   0.7941	      2.8370      1.3272    1.5389      0.4223
15			3.3023	   1.6784	      4.2281      2.7472    2.2982      1.0079
20			4.6425	   3.0033         5.9361      4.7462    3.1808      1.9556
25			6.1743	   4.6739         7.8859      7.0497    4.1535      3.1073
30			7.8579	   6.5590         9.9668      9.4274    5.1946      4.2868
35			9.6641	   8.5561         12.0978     11.7853   6.2779      5.4354
40			11.5635	   10.6030        14.2428     14.0439   7.3726      6.5550
45          13.5283    12.6693        16.3840     16.2052   8.4633      7.6562
50          15.5362    14.7423        18.5134     18.3187   9.5476      8.7454





   

==> Figs/data_Plot5_Javad.tex <==
SNR	       	Greedy	     	        Linear-eq   Linear-rand     	Linear								
0			0.7135					0.3889         0.0612          0.6695
5			1.3473				    0.7425         0.1633          1.2581
10			2.2018					1.2272	       0.3979          2.0300
15			3.3023					1.7197	       0.8607          3.0187
20			4.6425				    2.4699         1.5390          4.2450
25			6.1743					3.6239         2.2430          5.6891
30			7.8579			        5.1457         3.3170          7.3071
35			9.6641					6.9447         4.7895          9.0608
40			11.5635		            8.9060         6.5470          10.9183
45          13.5283                 10.9337        8.4835          12.8578
50          15.5362                 12.9863        10.5039         14.8513
    
 

==> Figs/data_Plot6J.tex <==
SNR	RsymL2G2K2t1cov		RsymLMMSEmultistreamL2G2K2t1				RsymLMMSEsinglestreamL2G2K2t1				RsymLMMSEmultistreamL8G4K3t1				RsymCovL8G4K3t1			RsymLMMSEsinglestreamL8G4K3t1				RsymproposedL8G4K4LMMSE				RsymCovL5G4K3t1			RsymproposedLMMSEL5G4K3t1				RsymproposedLMMSEsinglestreamL5G4K3t1			RsymproposedCovL8G4K4t1	
																																					
0	3.6949		3.6324					4.0999				13.1967				13.8776			13.1158				13.4936			10.8459			10.1912				10.5128406			14.94228889	
5	6.811		6.669					7.0231				23.4761				25.2802			22.1641				24.9845			19.8351			18.4914				18.67400687			27.37917778	
10	11.0363		10.8893					10.413				36.9815				40.3851			32.4828				40.6831			31.9366			29.0468				28.56133074			43.83483111	
15	16.3266		16.1615					13.999				53.7595				58.2191			43.3038				59.5164			46.4542			40.6405				39.20547288			63.20777778	
20	22.5407		22.4					17.6551				73.0311				78.225			54.252				80.2317			62.3754			52.5488				50.13539057			84.14940889	
25	29.3885		29.2652					21.3349				93.7875				99.533			65.1097				101.6557			78.8102			64.3329				61.08710934			105.6951569	
30	36.561		36.4331					25.0025				115.0608				121.4015			75.4295				122.9313			95.3402			75.5885				71.51098206			127.1925354	


==> Figs/data_Plot6J_1.tex <==
SNR	RsymL2G2K2t1cov		RsymLMMSEmultistreamL2G2K2t1				RsymLMMSEmultistreamL8G4K3t1				RsymCovL8G4K3t1			RsymproposedL8G4K4LMMSE				RsymCovL5G4K3t1			RsymproposedLMMSEL5G4K3t1				RsymproposedCovL6G4K3t1		RsymproposedCovL8G4K4t1				RsymproposedLMMSEL6G4K3t1	
																																
0	3.6949		3.6324					12.99958244				13.8776			13.4936			10.8459			10.1912				11.98615411			14.94228889			11.29802358	
5	6.811		6.669					22.92623884				25.2802			24.9845			19.8351			18.4914				21.89940687			27.37917778			19.89884353	
10	11.0363		10.8893					36.45770712				40.3851			40.6831			31.9366			29.0468				35.25402472			43.83483111			30.7681834	
15	16.3266		16.1615					53.27304337				58.2191			59.5164			46.4542			40.6405				50.99576337			63.20777778			43.03020121	
20	22.5407		22.4					72.48107396				78.225			80.2317			62.3754			52.5488				67.96777064			84.14940889			55.76402616	
25	29.3885		29.2652					93.36431831				99.533			101.6557			78.8102			64.3329				85.84500883			105.6951569			68.75105529	
30	36.561		36.4331					115.0374212				121.4015			122.9313			95.3402			75.5885				104.3980067			127.1925354			82.14918654	


==> Figs/data_Plot6_Javad.tex <==
SNR	       	Linear	  Linear-ZF         SIC       SIC-ZF	 NO-CC	   NO-CC-ZF					
0			0.7324	   0.3826         0.9937      0.5078    0.3322      0.0976
5			1.4743	   0.9694         2.0181      1.2734    0.6974      0.2733
10			2.5669	   2.0699	      3.4604      2.6807    1.2094      0.6626
15			4.0854	   3.7122	      5.3219      4.7226    1.8377      1.3096
20			5.9948	   5.7605         7.5371      7.1797    2.5511      2.1137
25		    8.1756	   8.0428         9.9768      9.8029    3.3090      2.9446
30			10.5121	   10.4398        12.5171     12.4507   4.0775      3.7512
35			12.9273	   12.8884        15.0883     15.0787   4.8416      4.5335
40			15.3812	   15.3611        17.6510     17.6671   5.5992      5.3006
45          17.8552    17.8452        20.2058     20.2257   6.3519      6.0588
50          20.3391    20.3304        22.7367     22.7513   7.1011      6.8117

  

==> Figs/data_Plot7_Javad.tex <==
SNR	   UL-DL-MJ   ZF-pl			Linear-test   Linear
0	   0.2038     0.0136          0.1361      0.2350
5	   0.3735     0.0410          0.2750      0.4376
10	   0.5800     0.1140          0.4671      0.7013
15	   0.8147	  0.2760          0.7049      1.0202
20	   1.0932     0.5599          0.9871      1.3924
25	   1.4378     0.9628          1.3084      1.8113
30	   1.8563     1.4571          1.6604      2.2703
35	   2.3410     2.0106          2.0399      2.7640
40	   2.8773     2.5965          2.4464      3.2881


    %0.2233
    %0.4205
    %0.6799
    %0.9937
    %1.3588
    %1.7691
    %2.2209
    %2.7097
    %3.2308


==> Figs/data_Plot8J.tex <==
TxAntenna		dofpropt1G4		dofWSAt1G4		dofpropt1G8		dofWSAt1G8		dofpropt1G12		dofWSAt1G12		dofpropt2G16		dofWSAt2G16		dofwsat0G16		dofpropt0G16
1		2		2		2		2		2		2		3		3		1		1
2		4		3		4		3		4		3		6		4		2		2
3		6		4		6		4		6		4		9		5		3		3
4		8		8		8		5		8		5		12		6		4		4
5		9		8		10		6		10		6		15		7		5		5
6		12		8		12		7		12		7		18		8		6		6
7		12		8		14		8		14		8		21		9		7		7
8		12		12		16		16		16		9		24		10		8		8
9		12		12		18		16		18		10		27		11		8		9
10		16		12		18		16		20		11		30		12		8		10
11		16		12		21		16		22		12		33		13		8		11
12		16		16		24		16		24		24		36		14		8		12
13		20		16		24		16		24		24		39		15		8		13
14		20		16		24		16		27		24		42		16		8		14
15		20		16		24		16		30		24		45		17		8		15
16		21		20		24		24		30		24		48		48		16		16
17		24		20		28		24		33		24		48		48		16		17
18		24		20		28		24		36		24		52		48		16		18
19		24		20		32		24		36		24		56		48		16		19
20		24		24		32		24		36		24		60		48		16		20
21		28		24		32		24		36		24		60		48		16		21
22		28		24		32		24		36		24		64		48		16		22
23		28		24		35		24		36		24		64		48		16		23
24		28		28		35		32		40		36		64		48		24		24
25		32		28		35		32		40		36		64		48		24		25
26		32		28		40		32		44		36		64		48		24		26
27		32		28		40		32		44		36		64		48		24		27
28		33		32		40		32		48		36		64		48		24		28
29		36		32		40		32		48		36		65		48		24		29
30		36		32		42		32		48		36		65		48		24		30
31		36		32		42		32		48		36		70		48		24		31
32		36		36		42		40		48		36		70		64		32		32
33		40		36		42		40		50		36		75		64		32		33
34		40		36		48		40		50		36		75		64		32		34
35		40		36		48		40		50		36		80		64		32		35
36		40		40		48		40		55		48		80		64		32		36
37		44		40		49		40		55		48		80		64		32		37
38		44		40		49		40		55		48		80		64		32		38
39		44		40		49		40		60		48		80		64		32		39
40		45		44		49		48		60		48		80		64		40		40
																				


==> Figs/data_Plot8J1.tex <==
RxAntenna		dofpropt2L20		dofWSAt2L20
2		24		24
4		28		28
6		36		30
8		40		32
10		45		40
12		48		36
14		56		42
16		60		48
18		60		54
20		60		60
22		60		60


==> Figs/data_Plot8J2.tex <==
t		DofwsaGL83	DofwsaGL85	DofwsaGL86	DofwsaLG87	DofwsaLG78	DofwsaLG68	DofwsaLG58	DofwsaLG38		DofpropGL83	DofpropGL85	DofpropGL86	DofpropLG87	DofpropLG78	DofpropLG68	DofpropLG58	DofpropLG38
																		
1		9	10	12	14	8	7	6	4		12	15	15	15	14	12	10	6
2		12	15	18	21	9	8	7	5		15	20	24	24	21	18	15	9
3		15	20	24	28	10	9	8	6		18	25	30	30	28	24	20	12
4		18	25	30	35	11	10	9	7		21	30	36	36	35	30	25	15
5		21	30	36	42	12	11	10	8		24	35	42	42	42	36	30	18
6		24	35	42	49	13	12	11	9		27	40	48	56	49	42	35	21
7		27	40	48	56	14	13	12	10		30	45	54	63	56	48	40	24
8		30	45	54	63	15	14	13	11		33	50	60	70	63	54	45	27
9		33	50	60	70	16	15	14	12		36	55	66	77	70	60	50	30
10		36	55	66	77	17	16	15	13		39	60	72	84	77	66	55	33
11		39	60	72	84	18	17	16	14		42	65	78	91	84	72	60	36
12		42	65	78	91	19	18	17	15		45	70	84	98	91	78	65	39
13		45	70	84	98	20	19	18	16		48	75	90	105	98	84	70	42
14		48	75	90	105	21	20	19	17		51	80	96	112	105	90	75	45
15		51	80	96	112	22	21	20	18		54	85	102	119	112	96	80	48
16		54	85	102	119	23	22	21	19		57	90	108	126	119	102	85	51
17		57	90	108	126	24	23	22	20		60	95	114	133	126	108	90	54
18		60	95	114	133	25	24	23	21		63	100	120	140	133	114	95	57
19		63	100	120	140	26	25	24	22		66	105	126	147	140	120	100	60
20		66	105	126	147	27	26	25	23		69	110	132	154	147	126	105	63

